A Study of Context Dependencies in Multi-page Product Search

In product search, users tend to browse results on multiple search result pages (SERPs) (e.g., for queries on clothing and shoes) before deciding which item to purchase. Users' clicks can be considered as implicit feedback which indicates their preferences and used to re-rank subsequent SERPs. Relevance feedback (RF) techniques are usually involved to deal with such scenarios. However, these methods are designed for document retrieval, where relevance is the most important criterion. In contrast, product search engines need to retrieve items that are not only relevant but also satisfactory in terms of customers' preferences. Personalization based on users' purchase history has been shown to be effective in product search. However, this method captures users' long-term interest, which does not always align with their short-term interest, and does not benefit customers with little or no purchase history. In this paper, we study RF techniques based on both long-term and short-term context dependencies in multi-page product search. We also propose an end-to-end context-aware embedding model which can capture both types of context. Our experimental results show that short-term context leads to much better performance compared with long-term and no context. Moreover, our proposed model is more effective than state-of-art word-based RF models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes


==> results.tex <==
%!TEX root=ProductSearch.tex
\section{Results and Discussion}
\label{sec:results}
%As we mentioned in Section \ref{subsec:baseline}, our proposed context-aware neural embedding model and all the baseline methods can be classified into three categories. 
%The first one is non-personalized retrieval models which rank items given queries without using users' information. PROD, RAND, POP, QL, and NEM fall into this category. These models can be used as the initial ranker for any queries, but they do not exploit information on the users' side. 
%The second type of rankers consider users' long-term interests together with queries and LC-RM3 is an example. This method conducts personalized ranking but can only be applied to users who appear in the training set. 
%The third type is feedback models which take users' clicks under the query in a search session as short-term context and this category includes SC-RM3 and our proposed SCEM. Different from the second type, users' identities are not needed. However, they can only be applied to search sessions where users click on results and only items from the second result page or later can be refined with the clicks. 

In this section, we show the performance of the four types of models mentioned in Section \ref{subsec:baseline}. 
First, we compare the overall retrieval performance of various types of models in Section \ref{subsec:overall_perf}. 
Then we further study the effect of queries, long-term context and embedding size on each model in the following subsections.

%TODO:some text introduce what this section is about
\begin{table*}
	\caption{Comparison of baselines and our short-term context embedding model (SCEM) on re-ranking when users paginate to the 2nd and 3rd page. The number is the relative improvement of each method compared with the production model (PROD)\protect\footnotemark. `$^-$' indicates significant worse of each baseline compared with SCEM `$^-$' in student t-test with $p \leq 0.001$. Note that difference larger than 3\% is approximately significant. The best performance in each column is marked in bold. }
	\label{tab:overallperf}
	%\large
	%    \addtolength{\tabcolsep}{3pt} 
	\scalebox{0.9}{    
	\begin{tabular}{  p{1.5cm} || r | r | r || r | r | r || r | r | r   }
	%\begin{tabular}{  p{1.5cm} | c || l || l ||  l || l | l | l || l || l ||  l | l | l  }
		\hline
		\multicolumn{10}{c}{Performance of Re-ranking from the 2nd Page} \\
		\hline
		& \multicolumn{3}{c||}{Toys \& Games} & \multicolumn{3}{c||}{Garden \& Outdoor} & \multicolumn{3}{c}{Cell Phones \& Accessories} \\
		\hline
		Model & $MAP$ & $MRR$ & $NDCG@10$ & $MAP$ & $MRR$ & $NDCG@10$ & $MAP$ & $MRR$ & $NDCG@10$ \\
		\hline
		\hline
		PROD & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ \\
		\hline
		RAND & -25.70\%$^{-}$ & -26.83\%$^{-}$ & -29.23\%$^{-}$ & -23.40\%$^{-}$ & -24.16\%$^{-}$ & -25.73\%$^{-}$ & -20.15\%$^{-}$ & -20.93\%$^{-}$ & -22.73\%$^{-}$ \\
		\hline
		POP & -15.82\%$^{-}$ & -15.90\%$^{-}$ & -17.87\%$^{-}$ & -9.38\%$^{-}$ & -9.51\%$^{-}$ & -9.55\%$^{-}$ & -8.54\%$^{-}$ & -8.25\%$^{-}$ & -11.12\%$^{-}$ \\
		\hline
		QL & -25.78\%$^{-}$ & -27.80\%$^{-}$ & -29.73\%$^{-}$ & -19.62\%$^{-}$ & -20.78\%$^{-}$ & -21.63\%$^{-}$ & -16.14\%$^{-}$ & -16.77\%$^{-}$ & -18.00\%$^{-}$ \\
		\hline
		QEM & -2.57\%$^{-}$ & -3.10\%$^{-}$ & -3.85\%$^{-}$ & +0.65\%$^{-}$ & -0.34\%$^{-}$ & +1.06\%$^{-}$ & +9.96\%$^{-}$ & +9.73\%$^{-}$ & +10.58\%$^{-}$ \\
		\hline
		\hline
		LCRM3 & -24.82\%$^{-}$ & -25.92\%$^{-}$ & -28.60\%$^{-}$ & -19.33\%$^{-}$ & -20.45\%$^{-}$ & -21.28\%$^{-}$ & -15.44\%$^{-}$ & -16.07\%$^{-}$ & -17.38\%$^{-}$ \\
		\hline
		LCEM & -2.57\%$^{-}$ & -3.10\%$^{-}$ & -3.85\%$^{-}$ & +0.65\%$^{-}$ & -0.34\%$^{-}$ & +1.06\%$^{-}$ & +9.96\%$^{-}$ & +9.73\%$^{-}$ & +10.58\%$^{-}$ \\
		\hline
		\hline
		SCRM3 & +12.93\%$^{-}$ & +9.63\%$^{-}$ & +9.53\%$^{-}$ & +25.15\%$^{-}$ & +23.01\%$^{-}$ & +23.15\%$^{-}$ & +18.65\%$^{-}$ & +16.77\%$^{-}$ & +17.11\%$^{-}$ \\
		\hline
		SCEM & \textbf{+26.59\%} & \textbf{+24.56\%} & \textbf{+26.20\%} & \textbf{+37.43\%} & \textbf{+35.16\%} & \textbf{+37.22\%} & \textbf{+48.99\%} & \textbf{+47.00\%} & \textbf{+50.18\%} \\
		\hline
		\hline
		LSCEM & \textbf{+26.59\%} & \textbf{+24.56\%} & \textbf{+26.20\%} & \textbf{+37.43\%} & \textbf{+35.16\%} & \textbf{+37.22\%} & \textbf{+48.99\%} & \textbf{+47.00\%} & \textbf{+50.18\%} \\
		\hline
		\hline
%		\multicolumn{10}{c}{Performance of Re-ranking from the 3rd Page} \\
%		\hline
%		& \multicolumn{3}{c||}{Toys \& Games} & \multicolumn{3}{c||}{Garden \& Outdoor} & \multicolumn{3}{c}{Cell Phones \& Accessories} \\
%		\hline
%		Model & $MAP$ & $MRR$ & $NDCG@10$ & $MAP$ & $MRR$ & $NDCG@10$ & $MAP$ & $MRR$ & $NDCG@10$ \\
%		\hline
%		\hline
%		PROD & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ & 0.00\%$^{-}$ \\
%		\hline
%		RAND & -15.45\%$^{-}$ & -17.97\%$^{-}$ & -18.96\%$^{-}$ & -12.29\%$^{-}$ & -13.71\%$^{-}$ & -13.97\%$^{-}$ & -8.75\%$^{-}$ & -10.05\%$^{-}$ & -9.55\%$^{-}$ \\
%		\hline
%		POP & -4.37\%$^{-}$ & -5.31\%$^{-}$ & -5.18\%$^{-}$ & 2.09\%$^{-}$ & 1.43\%$^{-}$ & 3.49\%$^{-}$ & -0.78\%$^{-}$ & -1.21\%$^{-}$ & -1.43\%$^{-}$ \\
%		\hline
%		QL & -14.87\%$^{-}$ & -18.31\%$^{-}$ & -19.20\%$^{-}$ & -9.15\%$^{-}$ & -10.97\%$^{-}$ & -10.37\%$^{-}$ & -4.05\%$^{-}$ & -5.21\%$^{-}$ & -3.62\%$^{-}$ \\
%		\hline
%		QEM & +12.83\%$^{-}$ & +11.07\%$^{-}$ & +14.13\%$^{-}$ & +15.82\%$^{-}$ & +14.42\%$^{-}$ & +19.32\%$^{-}$ & +28.85\%$^{-}$ & +27.60\%$^{-}$ & +33.92\%$^{-}$ \\
%		\hline
%		\hline
%		LCRM3 & -13.99\%$^{-}$ & -15.82\%$^{-}$ & -17.20\%$^{-}$ & -9.02\%$^{-}$ & -10.73\%$^{-}$ & -10.04\%$^{-}$ & -3.26\%$^{-}$ & -4.48\%$^{-}$ & -2.85\%$^{-}$ \\
%		\hline
%		LCEM & +12.83\%$^{-}$ & +11.07\%$^{-}$ & +14.13\%$^{-}$ & +15.82\%$^{-}$ & +14.42\%$^{-}$ & +19.32\%$^{-}$ & +28.85\%$^{-}$ & +27.60\%$^{-}$ & +33.92\%$^{-}$ \\
%		\hline
%		\hline
%		SCRM3 & +34.26\%$^{-}$ & +29.27\%$^{-}$ & +32.86\%$^{-}$ & +49.54\%$^{-}$ & +46.60\%$^{-}$ & +51.20\%$^{-}$ & +44.52\%$^{-}$ & +41.16\%$^{-}$ & +46.98\%$^{-}$ \\
%		\hline
%		SCEM & \textbf{+51.46\%} & \textbf{+47.57\%} & \textbf{+54.77\%} & \textbf{+63.79\%} & \textbf{+60.43\%} & \textbf{+67.79\%} & \textbf{+85.51\%} & \textbf{+81.72\%} & \textbf{+93.85\%} \\
%		\hline
%		\hline
%		LSCEM & \textbf{+51.46\%} & \textbf{+47.57\%} & \textbf{+54.77\%} & \textbf{+63.79\%} & \textbf{+60.43\%} & \textbf{+67.79\%} & \textbf{+85.51\%} & \textbf{+81.72\%} & \textbf{+93.85\%} \\
%		\hline
%		\hline
	\end{tabular}
	}
\end{table*}
\footnotetext{Due the confidentiality policy, the absolute value of each metric can not be revealed.}
\begin{comment}
%The original number is shown for Amazon Machine Learning Conference.
\begin{table*}
	\caption{Comparison of baselines and our short-term context embedding model (SCEM) on re-ranking when users paginate to the 2nd and 3rd page. The number is the relative improvement of each method compared with the production model (PROD)\protect\footnotemark. Significant differences of each baseline compared with SCEM are indicated with `*' in student t-test with $p \leq 0.005$. The best performance in each column is marked in bold. }
	\label{tab:overallperf}
	%\large
	%    \addtolength{\tabcolsep}{3pt} 
	%\scalebox{0.85}{    
	\begin{tabular}{  p{1.5cm} || r | r | r || r | r | r || r | r | r   }
		%\begin{tabular}{  p{1.5cm} | c || l || l ||  l || l | l | l || l || l ||  l | l | l  }
		\hline
		\multicolumn{10}{c}{Performance of Re-ranking from the 2nd Page} \\
		\hline
		& \multicolumn{3}{c||}{Toys \& Games} & \multicolumn{3}{c||}{Garden \& Outdoor} & \multicolumn{3}{c}{Cell Phones \& Accessories} \\
		\hline
		Model & $MAP$ & $MRR$ & $NDCG$ & $MAP$ & $MRR$ & $NDCG$ & $MAP$ & $MRR$ & $NDCG$ \\
		\hline
		PROD & 0.1245 & 0.1547 & 0.1584 & 0.1376 & 0.1482 & 0.1706 & 0.1335 & 0.1419 & 0.1654 \\ \hline
		RAND & 0.0925 & 0.1132 & 0.1121 & 0.1054 & 0.1124 & 0.1267 & 0.1066 & 0.1122 & 0.1278 \\ \hline
		POP & 0.1048 & 0.1301 & 0.1301 & 0.1247 & 0.1341 & 0.1543 & 0.1221 & 0.1302 & 0.1470 \\ \hline
		QL & 0.0924 & 0.1117 & 0.1113 & 0.1106 & 0.1174 & 0.1337 & 0.1120 & 0.1181 & 0.1356 \\ \hline
		QEM & 0.1213 & 0.1499 & 0.1523 & 0.1385 & 0.1477 & 0.1724 & 0.1468 & 0.1557 & 0.1829 \\ \hline
		LCRM3 & 0.0936 & 0.1146 & 0.1131 & 0.1110 & 0.1179 & 0.1343 & 0.1129 & 0.1191 & 0.1366 \\ \hline
		SCRM3 & 0.1406 & 0.1696 & 0.1735 & 0.1722 & 0.1823 & 0.2101 & 0.1584 & 0.1657 & 0.1937 \\ \hline
		SCEM & \textbf{0.1576} & \textbf{0.1927} & \textbf{0.1999} & \textbf{0.1891} & \textbf{0.2003} & \textbf{0.2341} & \textbf{0.1989} & \textbf{0.2086} & \textbf{0.2484} \\ \hline
		\hline
		\multicolumn{10}{c}{Performance of Re-ranking from the 3rd Page} \\
		\hline
		& \multicolumn{3}{c||}{Toys \& Games} & \multicolumn{3}{c||}{Garden \& Outdoor} & \multicolumn{3}{c}{Cell Phones \& Accessories} \\
		\hline
		Model & $MAP$ & $MRR$ & $NDCG$ & $MAP$ & $MRR$ & $NDCG$ & $MAP$ & $MRR$ & $NDCG$ \\
		\hline
		PROD & 0.0686 & 0.0885 & 0.0849 & 0.0765 & 0.0839 & 0.0916 & 0.0766 & 0.0826 & 0.0911 \\ \hline
		RANDOM & 0.0580 & 0.0726 & 0.0688 & 0.0671 & 0.0724 & 0.0788 & 0.0699 & 0.0743 & 0.0824 \\ \hline
		POP & 0.0656 & 0.0838 & 0.0805 & 0.0781 & 0.0851 & 0.0948 & 0.0760 & 0.0816 & 0.0898 \\ \hline
		QL & 0.0584 & 0.0723 & 0.0686 & 0.0695 & 0.0747 & 0.0821 & 0.0735 & 0.0783 & 0.0878 \\ \hline
		QEM & 0.0774 & 0.0983 & 0.0969 & 0.0886 & 0.0960 & 0.1093 & 0.0987 & 0.1054 & 0.1220 \\ \hline
		LCRM3 & 0.0590 & 0.0745 & 0.0703 & 0.0696 & 0.0748 & 0.0824 & 0.0741 & 0.0789 & 0.0885 \\ \hline
		SCRM3 & 0.0921 & 0.1144 & 0.1128 & 0.1144 & 0.1230 & 0.1385 & 0.1107 & 0.1166 & 0.1339 \\ \hline
		SCEM & \textbf{0.1039} & \textbf{0.1306} & \textbf{0.1314} & \textbf{0.1253} & \textbf{0.1346} & \textbf{0.1537} & \textbf{0.1421} & \textbf{0.1501} & \textbf{0.1766} \\ \hline
		\hline
	\end{tabular}
\end{table*}
\end{comment}


\subsection{Overall Retrieval Performance}
\label{subsec:overall_perf}
Table \ref{tab:overallperf} shows the performance of different methods on re-ranking items when users paginate to the second and third SERP for \textit{Toys \& Games, Garden \& Outdoor} and \textit{Cell Phones \& Accessories}. Among all the methods, SCEM and SCRM3 perform better than all the other baselines without using short-term context, including their corresponding retrieval baseline, QEM, and QL respectively, and PROD which considers many additional features, showing the effectiveness of incorporating short-term context. 

In contrast to the effectiveness of short-term context, long-term context does not help much when combined with queries alone or together with short-term context. LCRM3 outperforms QL on all the datasets by a small margin when users' historical purchases are used to represent their preferences. LCEM and LSCEM always perform worse than QEM and SCEM by incorporating long-term context with $\lambda_u > 0$. 
%So we did not show their performance in the table, and .
Note that since only a small portion of users in the test set appear in the training set, the re-ranking performance of most query sessions in the test set will not be affected. We will elaborate on the effect of long-term context in Section \ref{subsec:user_effect}. 
%(See Table \ref{tab:stats})

We found that neural embedding methods are more effective than word-based baselines. When implicit feedback is not incorporated, QEM performs significantly better than QL, sometimes even better than PROD. When clicks are used as context, with neural embeddings, SCEM is much more effective than SCRM3. This shows that semantic match is more beneficial than exact word match for top retrieved items in product search. In addition, these embeddings also carry the popularity information since items purchased more in the training data will get more gradients during training. Due to our model structure, there are also properties that the embeddings of items purchased under similar queries or context will be more alike compared with non-purchased items, and embeddings of clicked and purchased items are also similar. 

The relative improvement of SCEM and SCRM3 compared to the production model on Toys \& Games is less than the other two datasets. There are two possible reasons. 
First, the production model performs better on Toys \& Games, compared with Garden \& Outdoor, and Cell Phones \& Accessories, which can be seen from the larger advantages compared with random re-ranking. 
Second, 
% as shown in Table \ref{tab:stats}, 
the average clicks in the first two and three SERPs in Toys \& Games are less than the other two datasets \footnote{The specific number of average clicks in the datasets cannot be revealed due to the confidentiality policy. }, thus SCEM and SCRM3 can perform better with more implicit feedback information. 

\begin{figure*}
	\centering
	\begin{subfigure}{.25\textwidth}
		\centering
		\includegraphics[width=1.7in]{figures/lambda_c.pdf}
		\caption{$\lambda_c$}
		\label{fig:a}
	\end{subfigure}%
	\begin{subfigure}{.25\textwidth}
		\centering
		\includegraphics[width=1.7in]{figures/lambda_u.pdf}
		\caption{$\lambda_u$}
		\label{fig:b}
	\end{subfigure}%
	\begin{subfigure}{.25\textwidth}
		\centering
		\includegraphics[width=1.7in]{figures/lambda_u_seen.pdf}
		\caption{$\lambda_u$ on seen users}
		\label{fig:c}
	\end{subfigure}%
	\begin{subfigure}{.25\textwidth}
		\centering
		\includegraphics[width=1.7in]{figures/embed_size.pdf}
		\caption{Embedding size}
		\label{fig:d}
	\end{subfigure}%
	\caption{The effect of $\lambda_c$, $\lambda_u$, embedding size on the performance of each model in the collection of \textit{Toys \& Games} when re-ranking from the second SERP for the scenarios where users paginate to page 2.}
	\label{fig:param_effect}
\end{figure*}


The relative performance of all the other methods against PROD is better when re-ranking from page 2 compared with re-ranking from page 3 in terms of all three metrics. Several reasons are shown as follows. 
% The number of valid query sessions for re-ranking from the 3rd page is less than re-ranking from the 2nd page since there are fewer users paginating to page 3 than page 2 in the search log. The specific numbers are shown in Table \ref{tab:stats}. 
When purchases happen in the third page or later, it usually means users cannot find the ``right'' products in the first two pages, which further indicates the production model is worse for these query sessions. In addition, the ranking quality of PROD on the third page is worse than on the second page.  
Another reason that SCRM3 and SCEM improve more upon PROD when re-ranking from page 3 is that more context becomes available with clicks collected in the second page and makes the user preference model more robust. 

QL performs similarly to RAND on Toys \& Games and a little better than RAND on Garden \& Outdoor, and Cell Phones \& Accessories, which indicates that relevance captured by exact word matching is not the key concern in the rank lists of the production model.
% that most top-ranked items retrieved by the production model cover the query words. 
In addition, most candidate products are consistent with the query intent but the final purchase depends on users' preference. Popularity, as an important factor that consumers will consider, can improve the performance upon QL. However, it is still worse than the production model most of the time.
% since it is only one of the many features the product model covers. 


\subsection{Effect of Short-term Context} %on Context-aware Product Search
\label{subsec:query_effect}
%figure of parameter sensitivity
We investigate the influence of short-term context by varying the value of $\lambda_c$ with $\lambda_u$ set to 0. The performance of SCRM3 and SCEM varies as the interpolation coefficient of short-term context changes since only these two methods utilize the clicks.
 Since re-ranking from the second or third pages on \textit{Toys \& Games, Garden} and \textit{Mobile} all show similar trends, we only report performance of each method in the setting of re-ranking from second pages on \textit{Toys \& Games}, which is shown in Figure \ref{fig:a}.  
% The value of $MAP$ only changes for SC-RM3 and SCEM when different $\lambda_q$ are used since only these two methods utilize the click information.  
Figure \ref{fig:a} shows that as the weight of clicks is set larger, the performance of SCRM3 and SCEM goes up consistently. When $\lambda_c$ is set to 0, SCRM3 and SCEM degenerate to QL and QEM respectively which do not incorporate short-term context. From another perspective, 
SCRM3 and SCEM degrade in performance as we increase the weight on queries. 
%the more weight queries take up, the worse performance SCRM3 and SCEM will produce. 
For exact word match based methods, more click signals lead to more improvements for SCRM3, which is also consistent with the fact that QL performs similarly to RAND by only considering queries.
For embedding-based methods which capture semantic match and popularity, QEM with queries alone performs similarly to PROD but much better when more context information is incorporated in SCEM. This indicates that users' clicks already cover the query intent, and also contain additional users' preference information. 

\subsection{Effect of Long-term Context} %  on Context-aware Product Search
\label{subsec:user_effect}
Next we study the effect of long-term context indicated by users' global representations $\mathcal{E}(u)$ both with and without incorporating short-term context. QEM and LCRM3 only use queries and user historical transactions for ranking; LSCEM uses long and short-term context ($\lambda_u+\lambda_c$ is fixed as 1 since we found that query embeddings do not contribute to the re-ranking performance when short-term context is incorporated).
% on each model as a personalized preference indicated by long-term interest. 
%We vary the value of $\lambda_u$ for CNEM, NEM and L-RM3 to see the effect of users' long-term interest on retrieval when the short-term context is considered (for CNEM) or not (for L-RM3 and NEM). 
\textit{Toys \& Games} is used again to show the sensitivity of each model in terms of $\lambda_u$ under the setting of re-ranking from the second page. Since there are users in the test set which never appear in the training set, $\lambda_u$ does not take effect due to the null representations for these unknown users. 
% for the unknown users, 
% In Toys \& Games, only 8855 session-query pairs are from users who appear in both training and test set, which account for about 13\% of all the available query sessions of the test set (See Table \ref{tab:stats}). 
In Toys \& Games, only about 13\% of all the query sessions in the test set are from users who also appear in the training set.
The performance change on the entire test set will be smaller due to the low proportion the models can effect in the test set, so we also include the performance of each model on the subset of data entries associated with users seen in the training set. Figure \ref{fig:b} and \ref{fig:c} show how each method performs on the whole test set and the subset respectively with different $\lambda_u$. 

Figure \ref{fig:b} and \ref{fig:c} show that for LSCEM, as $\lambda_u$ becomes larger,
%which corresponds to the third sub-figure in Figure \ref{fig:depend}, 
performance goes down. This indicates that when short-term contexts are used, users' embeddings act like noise and drag down the re-ranking performance. 
$\lambda_u$ has different impacts on the models not using clicks. For LCRM3, when we zoom in to only focus on users that appear in the training set, the performance changes and the superiority over QL are more noticeable. The best value of $MAP$ is achieved when $\lambda_u=0.8$, which means long-term context benefit word-based models with additional information, which can be helpful for solving the word mismatch problem. In contrast, for LCEM, with non-zero $\lambda_u$, it performs worse than only considering queries. Embedding models already capture semantic similarities between words. In addition, as we mentioned in Section \ref{subsec:overall_perf}, they also carry information about popularity since the products purchased more often under the query will get more credits during training. Another possible reason is that the number of customers with sessions of similar intent is low so that the user embedding is misguiding the query sessions.
Thus, users' long-term interests do not bring additional information to further improve LCEM on the collections. 

This finding is different from the observation in HEM proposed by \citet{ai2017learning}, which incorporates user embeddings as users' long-term preferences and achieves superior performance compared to not using user embeddings. 
%The inconsistent conclusions are probably because the datasets we used have different properties. 
We hypothesize that this inconsistent finding is due to the differences in datasets.
HEM was experimented on a dataset that is heavily biased to users with multiple purchases and under a rather simplistic assumption of query generation, where the terms from the category hierarchy of a product are concatenated as the query string. Their datasets contain only hundreds of unique queries and tens of thousands items that are all purchased by multiple users. 
In contrast, we experimented on the real queries and corresponding user behavior data extracted from search log. The number of unique queries and items in our experiments are hundreds times larger than in their dataset. There is also little overlap of users in the training and test set in our datasets, while in their experiments, all the users in the test set are shown in the training set. 
%From the above, we can infer that the number of customers with similar intents in training and test set are much less in our dataset compared in theirs, which causes that user embeddings do not benefit LCEM and LSCEM in our experiments.
 
%I think the number of customers with sessions of similar intent is low and that’s why the user embedding is misguiding the search session in almost all cases. We cannot reveal the numbers here but we can describe this a little. We should also discuss about your HEM, as an example of LCEM, that achieved superior performance. We can perhaps attribute its performance to the use of a dataset that is heavily biased to users with multiple purchases and under a rather simplistic assumption of query generation.


%\textbf{Comparison of Methods With and Without Context}

\subsection{Effect of Embedding Size}
\label{subsec:embed_size}
Figure \ref{fig:d} shows the sensitivity of each model in terms of embedding size on \textit{Toys \& Games}, which presents similar trends to the other two datasets. Generally, SCEM and QEM are not sensitive to the embedding size as long as it is in a reasonable range. 
%When it is set to 50, the values of $MAP$ for QEM and SCEM drop a little amount. When it is more than 50, not many differences appear. 
To keep the model effective and simple, we use 100 as the embedding size and report experimental results under this setting in Table \ref{tab:overallperf} and the other figures. 
%case analysis ?
%\textbf{Long-term Interest vs Short-term Context}

%\textbf{Personalization vs Non-personalization}

